A Minimal OO Calculus for Modelling Biological Systems

In this paper we present a minimal object oriented core calculus for modelling the biological notion of type that arises from biological ontologies in formalisms based on term rewriting. This calculus implements encapsulation, method invocation, subtyping and a simple formof overriding inheritance, and it is applicable to models designed in the most popular term-rewriting formalisms. The classes implemented in a formalism can be used in several models, like programming libraries.

==> eptcsdata.tex <==
\providecommand{\firstpage}{50}
\providecommand{\publicationstatus}{Ion Petre and Erik De Vink (Eds.): Third International Workshop on\\ Computational Models for Cell Processes (CompMod 2011)\\
EPTCS 67, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.67.6}{10.4204/EPTCS.67.6}}

